A Tight Theory of Error Feedback Algorithms in Distributed Optimization

Communication costs are a major bottleneck in distributed learning and first-order optimization. A common approach to alleviate this issue is to compress the gradient information exchanged between agents. However, such compression typically degrades the convergence guarantees of gradient-based methods. Error feedback mechanisms provide a simple and computationally cheap remedy for this issue, but numerous variants have been proposed, and their relative performance remains poorly understood. This paper provides tight convergence analyses for two of the main error-feedback algorithms from the literature, the classic Error Feedback method (EF) and Error Feedback 21 (EF21), by identifying optimal step-size choices and constructing optimal Lyapunov functions tailored to each method. The results hold independently of the number of agents and recover the known best guarantees possible in the single-agent regime.

==> certified.tex <==
\ProvidesFile{certified.tex}[2025/10/17 Certified block (brace+box)]
\usepackage{stmaryrd}
\usepackage{fontawesome5}

\RequirePackage{xparse}
\RequirePackage{etoolbox}
\RequirePackage{graphicx}
\RequirePackage{pgfkeys}
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathreplacing,calc}

\makeatletter
\@ifpackageloaded{tcolorbox}{}{\RequirePackage{tcolorbox}}
\tcbuselibrary{skins,breakable}
\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\@ifpackageloaded{footnotehyper}{}{\RequirePackage{footnotehyper}} %
\@ifpackageloaded{xcolor}{}{\RequirePackage{xcolor}}
\makeatother
\makesavenoteenv{tcolorbox}  %

\IfFileExists{currfile.sty}{%
  \RequirePackage{currfile}
  \makeatletter \edef\certblockdir{\currfiledir} \makeatother
  \graphicspath{{\certblockdir}{./}}
}{}

\newlength\CertifiedBraceGap    \setlength\CertifiedBraceGap{0.9em}
\newlength\CertifiedBraceRise   \setlength\CertifiedBraceRise{4pt}
\newcommand\CertifiedBraceWidth{1pt}
\newcommand\CertifiedBraceAmp{5pt}
\newcommand\CertifiedBraceColor{blue}

\pgfkeys{
  /certblock/.is family,
  /certblock/.cd,
  cas/.initial=,
  pep/.initial=,
  style/.initial=brace,      %
  box/.code   = \pgfkeysalso{/certblock/style=box},
  brace/.code = \pgfkeysalso{/certblock/style=brace},
  badgeheight/.initial=1.0em,
}

\newcommand*\certblockcas{}
\newcommand*\certblockpep{}
\newcommand*\certblockstyle{brace}

\newcommand*\certblockParse[1]{%
  \pgfkeys{/certblock/.cd, cas=, pep=, style=brace, badgeheight=1.0em}%
  \pgfkeys{/certblock/.cd, #1}%
  \pgfkeysgetvalue{/certblock/cas}{\certblockcas}%
  \pgfkeysgetvalue{/certblock/pep}{\certblockpep}%
  \pgfkeysgetvalue{/certblock/style}{\certblockstyle}%
}

\newcommand*\certcasiconfile{CAS.pdf}
\newcommand*\certcasbadgefile{CAS_inv.pdf}

\newcommand*\certblockicons{%
  \begingroup\setlength{\fboxsep}{0pt}%
  \def\out{}%
  \ifdefempty{\certblockcas}{}{%
    \edef\out{\out\noexpand\href[pdfnewwindow=true]{\certblockcas}{\noexpand\raisebox{-0.2ex}{\noexpand \includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{\certcasiconfile}}}}%
  }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\out}{}{\edef\out{\out\noexpand\hspace{0.4em}}}%
    \edef\out{\out\noexpand\href[pdfnewwindow=true]{\certblockpep}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{PEP.pdf}}}}%
  }%
  \out
  \endgroup
}

\newcommand*\certblockbadge{%
  \begingroup
  \def\result{external sources}%
  \ifdefempty{\certblockcas}{}{ \def\result{CAS} }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\certblockcas}{\def\result{PEP}}{\def\result{CAS \& PEP}}%
  }%
  \result
  \endgroup
}


\newcommand*\CertifiedFrameColor{green!75!black}
\newcommand*\CertifiedBackColor{green!12}
\definecolor{CertifiedHeaderGreen}{HTML}{258E58}
\newcommand*\CertifiedTitleBack{CertifiedHeaderGreen}
\newcommand*\CertifiedTitleTextColor{white}
\makeatletter
\@ifundefined{color@ForestGreen}{\definecolor{ForestGreen}{rgb}{0.13,0.55,0.13}}{}
\makeatother
\newcommand*\CertifiedBadgeFill{none}
\newcommand*\CertifiedBadgeDraw{none}
\newcommand*\CertifiedBadgeTextColor{black}
\newcommand*\CertifiedBadgeFontSize{\scriptsize}
\newcommand*\CertifiedBadgeInnerX{4pt}
\newcommand*\CertifiedBadgeInnerY{2pt}

\pgfkeys{ /certblock/.cd, titletextcolor/.initial=} %

\newcommand*\CertifiedArc{6pt} %
\newcommand*\CertifiedRightArc{2pt} %
\newcommand*\CertifiedChipOffsetX{0pt}
\newcommand*\CertifiedChipOffsetY{0pt}
\newcommand*\CertifiedBadgeOffsetX{4pt}
\newcommand*\CertifiedBadgeOffsetY{0pt}
\newcommand*\CertifiedBadgeRightInset{0pt}

\newcommand{\certExtIcon}{%
  \raisebox{0.15ex}{\scalebox{0.85}{\faIcon{external-link-alt}}}%
}
\newcommand{\certBadgeContent}{%
  {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize
  CAS\hspace{0.4em}\certExtIcon}%
}
\newcommand*\certblockRenderBox[1]{%
  \newif\ifcertblockhasicons
  \certblockhasiconsfalse
  \ifdefempty{\certblockcas}{}{ \certblockhasiconstrue }%
  \ifdefempty{\certblockpep}{}{ \certblockhasiconstrue }%

  \edef\certblocktitletext{\noexpand\emph{Certified using WolframScript}}%

  \def\certblocktitlecolor{\CertifiedTitleTextColor}%
  \pgfkeysgetvalue{/certblock/titletextcolor}{\certblocktitletextcolor}%
  \ifdefempty{\certblocktitletextcolor}{}{\edef\certblocktitlecolor{\certblocktitletextcolor}}%

  \begin{tcolorbox}[
      enhanced,
      arc=\CertifiedArc,
      width=\linewidth,
      boxrule=0pt, %
      colframe=\CertifiedFrameColor,
      colback=\CertifiedBackColor,
      left=6pt,right=6pt,top=16pt,bottom=6pt,
      overlay={%
        \node[inner xsep=6pt, inner ysep=2pt,
          anchor=north west, outer sep=0pt,
        opacity=0] (certchip)
        at ([xshift=\CertifiedChipOffsetX,yshift=\CertifiedChipOffsetY]interior.north west)
        {\certblocktitletext};
        \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
        (certchip.north west) rectangle (certchip.south east);
        \path[fill=\CertifiedTitleBack, draw=none]
        (certchip.south west) rectangle ++(\CertifiedArc,\CertifiedArc);
        \begin{scope}
          \clip (certchip.center |- certchip.north east)
          rectangle
          (certchip.south east);
          \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
          (certchip.north west) rectangle (certchip.south east);
        \end{scope}
        \node[anchor=north west, outer sep=0pt,
        text=\certblocktitlecolor, font=\itshape]
        at (certchip.north west) {\certblocktitletext};
        \ifcertblockhasicons
        \ifdefempty{\certblockcas}{%
          \node[anchor=east, outer sep=0pt]
          at ([xshift=-\CertifiedBadgeRightInset, yshift=\CertifiedBadgeOffsetY]interior.north east |- certchip.east)
          {\begingroup\color{\CertifiedBadgeTextColor}\certblockiconsbadge\endgroup};
        }{%
          \begin{scope}
            \coordinate (badgeTR) at ([xshift=-\CertifiedBadgeRightInset]interior.north east);
            \coordinate (badgeBR) at ([xshift=-\CertifiedBadgeRightInset]interior.south east |- certchip.south);
            \node[anchor=base east, inner sep=0pt, outer sep=0pt, opacity=0] (castxt)
            at ([xshift=-\CertifiedBadgeRightInset-\CertifiedBadgeInnerX]interior.north east |- certchip.base east)
            {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize \certBadgeContent};
            \coordinate (badgeLX) at ([xshift=-\CertifiedBadgeInnerX]castxt.west);
            \coordinate (badgeTL) at (badgeLX |- certchip.north);
            \coordinate (badgeBL) at (badgeLX |- certchip.south);
            \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
            (badgeTL) rectangle (badgeBR);
            \begin{scope}
              \clip (badgeTL) rectangle (castxt.center |- badgeBR);
              \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
              (badgeTL) rectangle (badgeBR);
            \end{scope}
            \path[fill=\CertifiedTitleBack, draw=none]
            (badgeBR) rectangle ++(-\CertifiedArc,\CertifiedArc);
            \node[anchor=base east, inner sep=0pt, outer sep=0pt]
            at (castxt.base east)
            {\href[pdfnewwindow=true]{\certblockcas}{\textcolor{\CertifiedTitleTextColor}{\fontfamily{phv}\selectfont\CertifiedBadgeFontSize \certBadgeContent}}};
          \end{scope}
        }%
        \fi
      },
    ]#1
  \end{tcolorbox}%
}

\newcommand*\certblockRenderBrace[1]{%
  \begin{tcolorbox}[
      enhanced, blanker,
      left=0pt, right=0pt, top=0pt, bottom=0pt,
      boxsep=0pt, width=\linewidth,
      before upper=\setlength{\parindent}{0pt},
      overlay={%
        \draw[
          draw=\CertifiedBraceColor, line width=\CertifiedBraceWidth,
          decorate, decoration={brace,mirror,amplitude=\CertifiedBraceAmp}
        ]
        ([xshift=-\CertifiedBraceGap, yshift=\CertifiedBraceRise]frame.north west)
        --
        ([xshift=-\CertifiedBraceGap, yshift=-\CertifiedBraceRise]frame.south west)
        node[midway, anchor=east, xshift=-0.4em]{\certblockicons};
      }
    ]#1
  \end{tcolorbox}%
}

\NewDocumentCommand{\certifiedbox}{ O{} +m }{%
  \certblockParse{#1}%
  \certblockRenderBox{#2}%
}

\NewDocumentCommand{\certifiedblock}{ O{} +m }{%
  \certblockParse{#1}%
  \ifdefstrequal{\certblockstyle}{box}{%
    \certblockRenderBox{#2}%
  }{%
    \certblockRenderBrace{#2}%
  }%
}

\newcommand*\certlabelbox[1]{%
  \tikz[baseline=(txt.base)]{
    \node[inner xsep=\CertifiedBadgeInnerX, inner ysep=\CertifiedBadgeInnerY, outer sep=0pt,
    anchor=base west, opacity=0] (txt) {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize #1};
    \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedRightArc]
    (txt.north west) rectangle (txt.south east);
    \begin{scope}
      \clip (txt.center |- txt.north east) rectangle (txt.south east);
      \path[fill=\CertifiedTitleBack, draw=none, rounded corners=\CertifiedArc]
      (txt.north west) rectangle (txt.south east);
    \end{scope}
    \path[fill=\CertifiedTitleBack, draw=none]
    (txt.south east) rectangle ++(-\CertifiedArc,\CertifiedArc);
    \node[anchor=base west, outer sep=0pt, text=\CertifiedTitleTextColor]
    at (txt.base west) {\fontfamily{phv}\selectfont\CertifiedBadgeFontSize #1};
  }%
}

\newcommand*\certcasbox{\certlabelbox{CAS}}


\makeatletter
\@ifpackageloaded{thmtools}{}{%
  \RequirePackage{thmtools}
  \RequirePackage{thm-restate}
}
\@ifpackageloaded{xparse}{}{\RequirePackage{xparse}}
\@ifpackageloaded{pgfkeys}{}{\RequirePackage{pgfkeys}}
\@ifpackageloaded{etoolbox}{}{\RequirePackage{etoolbox}}
\@ifpackageloaded{graphicx}{}{\RequirePackage{graphicx}}
\makeatother

\providecommand\certhref[2]{#2}%
\makeatletter
\@ifpackageloaded{hyperref}{%
  \renewcommand\certhref[2]{\href[pdfnewwindow=true]{#1}{#2}}%
}{%
  \AtBeginDocument{%
    \@ifpackageloaded{hyperref}{\renewcommand\certhref[2]{\href[pdfnewwindow=true]{#1}{#2}}}{}%
  }%
}
\providecommand\cert@href[2]{\certhref{#1}{#2}}
\makeatother

\makeatletter

\newif\ifcertthm@cas
\newif\ifcertthm@pep

\providecommand*\certthmcas{}
\providecommand*\certthmpep{}
\providecommand*\certthmbadgeheightraw{1.0em}
\@ifundefined{certthmbadgeheight}{\newlength\certthmbadgeheight}{}

\pgfkeys{/certthm/.is family, /certthm,
  cas/.code={
    \pgfutil@ifempty{#1}{%
      \certthm@casfalse \def\certthmcas{}%
    }{%
      \certthm@castrue  \def\certthmcas{#1}%
    }%
  },
  pep/.code={
    \pgfutil@ifempty{#1}{%
      \certthm@pepfalse \def\certthmpep{}%
    }{%
      \certthm@peptrue  \def\certthmpep{#1}%
    }%
  },
  badgeheight/.code={
    \pgfutil@ifempty{#1}{%
      \def\certthmbadgeheightraw{1.0em}%
    }{%
      \def\certthmbadgeheightraw{#1}%
    }%
  },
}

\providecommand*\certthmParse{}%
\renewcommand*\certthmParse[1]{%
  \certthm@casfalse \certthm@pepfalse
  \def\certthmcas{}%
  \def\certthmpep{}%
  \def\certthmbadgeheightraw{1.0em}%
  \pgfkeys{/certthm/.cd, #1}%
  \setlength{\certthmbadgeheight}{\certthmbadgeheightraw}%
}

\newcommand{\certcenterimg}[1]{%
  \raisebox{.5\dimexpr\ht\strutbox - \dp\strutbox - \certthmbadgeheight\relax}%
  [\ht\strutbox][\dp\strutbox]{%
  \includegraphics[height=\certthmbadgeheight]{#1}}%
}

\makeatletter
\providecommand*\certthmicons{}%
\renewcommand*\certthmicons{%
  \begingroup
  \def\certthmhasicon{}%
  \ifcertthm@cas
  \def\certthmhasicon{1}%
  \certhref{\certthmcas}{\certcenterimg{CAS.pdf}}%
  \fi
  \ifcertthm@pep
  \ifcertthm@cas\hspace{0.4em}\fi
  \def\certthmhasicon{1}%
  \certhref{\certthmpep}{\certcenterimg{PEP.pdf}}%
  \fi
  \endgroup
}

\newcommand*\certblockiconsbadge{%
  \begingroup\setlength{\fboxsep}{0pt}%
  \def\out{}%
  \ifdefempty{\certblockcas}{}{%
    \edef\out{\out\noexpand\href[pdfnewwindow=true]{\certblockcas}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{\certcasbadgefile}}}}%
  }%
  \ifdefempty{\certblockpep}{}{%
    \ifdefempty{\out}{}{\edef\out{\out\noexpand\hspace{0.4em}}}%
    \edef\out{\out\noexpand\href[pdfnewwindow=true]{\certblockpep}{\noexpand\raisebox{-0.2ex}{\noexpand\includegraphics[height=\pgfkeysvalueof{/certblock/badgeheight}]{PEP.pdf}}}}%
  }%
  \out
  \endgroup
}
\makeatother
\makeatletter
\NewDocumentEnvironment{certified}{ O{} m m O{} +b }{%
  \certthmParse{#1}%
  \begingroup
  \let\cert@orig@begintheorem\@begintheorem
  \def\@begintheorem##1##2[##3]{%
    \thm@headpunct{.\hspace{0.4em}\certthmicons}%
    \def\thmheadnl{\newline}%
    \thm@headsep=0pt\relax
    \cert@orig@begintheorem{##1}{##2}[##3]%
  }%
  \begin{restatable}[#4]{#2}{#3}%
    \ignorespaces#5%
  \end{restatable}%
  \endgroup
}{}
\makeatother


\RequirePackage{graphicx} %

\newcommand{\certnoticeheight}{2.0em} %
\newcommand{\certnoticesep}{2em}      %
\newcommand{\certnoticevspace}{-2em}  %

\newcommand{\makecertificatenotice}{%
  \vspace*{\certnoticevspace}%
  \begin{center}
    \emph{Proof certificates are annotated using\footnote{We generate certificates of validity using a Computer Algebra System (CAS, via WolframScript) and Performance Estimation Problems (PEP). CAS annotations mark partial verification of proof identities, whereas PEP annotations indicate full verification of the statement. Each annotation links to the corresponding file in our GitHub repository}}%
    \par
    \includegraphics[height=\certnoticeheight]{CAS.pdf}\hspace{\certnoticesep}%
    \includegraphics[height=\certnoticeheight]{PEP.pdf}%
  \end{center}%
}

\newtcolorbox{caspara}[1][]{%
  breakable,
  enhanced,
  before skip=0pt,
  after skip=4pt,
  colback=\CertifiedBackColor,
  colframe=ForestGreen,
  arc=0pt,
  outer arc=0pt,
  title=Remark: proof certificates,
  fonttitle=\bfseries\sffamily,
  colbacktitle=ForestGreen,
  attach boxed title to top left={},
  boxed title style={
    enhanced,
    skin=enhancedfirst jigsaw,
    arc=3pt,
    bottom=0pt,
    interior style={fill=ForestGreen}
  }
}
\makesavenoteenv{caspara}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

